Statistical Nonlocality of Dynamically Coherent Structures

We introduce a class of stochastic advection problems amenable to analysis of turbulent transport. The statistics of the flow field are represented as a continuous time Markov process, a choice that captures the intuitive notion of turbulence as moving from one coherent structure to another. We obtain closed form expressions for the turbulent transport operator without invoking approximations. We recover the classical estimate of turbulent transport as a diffusivity tensor, the components of which are the integrated auto-correlation of the velocity field, in the limit that the operator becomes local in space and time.

==> Sections/old_alternative_computation.tex <==
\section{Continuum Formulation}
\label{continuum_formulation}
A numerical disrectization of the advection diffusion equation
\begin{align}
\partial_t \theta + \bm{u} \cdot \nabla \theta &= D \theta + s
\end{align}
is of the form
\begin{align}
\partial_t \theta_i + \sum_{jk} a_{ijk}u_j \theta_k &= \sum_{j} L_{ij} \theta_j + s_i
\end{align}
Thus the master equation for the discretization is 
\begin{align}
    \partial_t \rho &= \sum_{i} \frac{\partial}{\partial \theta_i } \left( \left[ \sum_{jk} a_{ijk}u_j \theta_k - \sum_{j} L_{ij} \theta_j - s_i\right] \rho \right) + T_{\bm{u}}[\rho]
\end{align}
where $T$ is a linear operator that denotes the transition probability of the stochastic variable $\bm{u}$. 

Here we have flattened all dimensions to a single index. 
We obtain the form in the text by multiplying the expression by $\Delta \bm{x}_i / \Delta \bm{x}_i$ where $\Delta \bm{x}_i$ is a volume element at location $i$ to get
\begin{align}
    \partial_t \rho &= \sum_{i}\Delta \bm{x}_i \frac{1}{\Delta \bm{x}_i} \frac{\partial}{\partial \theta_i } \left( \left[ \sum_{jk} a_{ijk}u_j \theta_k - \sum_{j} L_{ij} \theta_j - s_i\right] \rho \right) + T_{\bm{u}}[\rho]
\end{align}
which upon taking limits yields (using the naive thought process, product of limits is limit of products) 
\begin{align}
    \sum_{i}\Delta \bm{x} &\overset{``\text{lim}"}{ = } \int d \bm{x}  
    \\
    \frac{1}{\Delta \bm{x}_i } \frac{\partial}{\partial \theta_i } &\overset{``\text{lim}"}{ = } \frac{\delta}{\delta \theta (\bm{x} )}
    \\
    \left[ \sum_{jk} a_{ijk}u_j \theta_k - \sum_{j} L_{ij} \theta_j - s_i\right] 
    &\overset{``\text{lim}"}{ = } 
    \bm{u} \cdot \nabla \theta - D \theta - s
    \\
    \partial_t \rho &= \int d \bm{x} \frac{\delta}{\delta \theta (\bm{x} )} \left( \left[ \bm{u} \cdot \nabla \theta - D \theta - s \right] \rho  \right) + T_{\bm{u}}[\rho]
\end{align}
where $\bm{x}$ is a continuous index. (Perhaps change $\rho$ after the limit to something else? or do something like $\rho^i$ ? ). Perhaps mention $d \bm{\theta} \rightarrow \mathcal{D}[\theta]$




We start by writing the equation for the statistics of Equations \ref{stochastic_system_theta} and \ref{stochastic_system_u}. 


\begin{align}
\label{fokkerp_eqn}
\partial_t \rho_m &= -\int d\mathbf{x} \frac{\delta}{\delta \theta (\bm{x}) }\left( \left[  - \nabla \cdot \left( \mathbf{u}_m \theta - \kappa \nabla \theta \right)  + s \right] \rho_m \right) + \sum_n T_{mn} \rho_n
\end{align}
where the Louiville operator $\int d\mathbf{x} \frac{\delta}{\delta \theta }$ is the functional derivative equivalent of a divergence and $\rho_n[\theta, t]$ is the probability density at time $t$. 

To obtain an effective equation for $\langle \theta \rangle$ we must first calculate the intermediary quantities
\begin{align}
P_m \equiv \int \mathcal{D}[\theta]  \rho_m \text{ and } \Theta_m \equiv \int \mathcal{D}[\theta] \theta \rho_m 
\end{align}
for each index $m$. Here we have introduced the path integrals $\int \mathcal{D}[\theta]$ where the volume element $\mathcal{D}[\theta]$ is an infinitesmal volume of function space and the integral is a rule to integrate over all functions. The $P_m$ is the distribution of the flow statistics and the $\Theta_m$ is the conditional mean. 

The equation for $P_m$ is
\begin{align}
    \partial_t P_m &= \sum_n T_{mn }P_n 
\end{align}
and $\Theta_m$ is 
\begin{align}
\label{statistics}
    \partial_t \Theta_m + \nabla \cdot \left( \bm{u}_m \Theta_m - \kappa \nabla \Theta_m \right)  &= P_m s(x) + \sum_n T_{mn} \Theta_n
\end{align}
By applying the summation operator $\sum_m$ on \ref{statistics} we obtain
\begin{align}
\label{mean_statistics}
    \partial_t \sum_m \Theta_m + \nabla \cdot \sum_m \left( \bm{u}_m \Theta_m - \kappa \nabla \Theta_m \right)  &= s(x)
\end{align}
where we made use of the identity $\sum_{m} T_{mn} = 0$. We identify \eref{statistics} with \eref{mean_equations} via the identities $\langle \theta \rangle = \sum_m \Theta_m$ and $\langle \bm{u} \theta \rangle = \sum_m \bm{u}_m \Theta_m$; however, unlike \eref{mean_equations}, \eref{statistics} has an explicit dependence on the ``perturbation variables" as they relate to the statistical distribution of $\bm{u}$ and thus offer a useful relation for directly solving for the statistics. The large system of coupled perturbution variable will be related to the koopman modes associated with non-zero eigenvalues of the transition operator $T$.

Given that we are in state $n$ we define the transition probability from state $n -> m$ as $T_{nm}$. By expanding in terms of the eigenfunctions of the transition probability we order then in terms of the lowest mode and the highest mode. By comparison with \ref{mean_equations} we see that the equation for the zero'th eigenfunction is in exact correspondence. Hence we can interpret the term in parenthesis as the eddy-flux that we have sought.


At any rate let's go back to the discrete system and look at the moment equations
\begin{align}
    \partial_t \rho &= \sum_{i} \frac{\partial}{\partial \theta_i } \left( \left[ \sum_{jk} a_{ijk}u_j \theta_k - \sum_{j} L_{ij} \theta_j - s_i\right] \rho \right) + T_{\bm{u}}[\rho]
\end{align}
Integrating with respect to $d \bm{\theta}$ just yields the marginal distribution for the velocity field. 

Multiplying through by $\theta^j$ and doing the usual stuff yields 

\begin{align}
    \partial_t \Theta^i + \sum_{jk} a_{ijk}u_j \Theta^k &=  \sum_{j} L_{ij} \Theta^j - s_i + T_{\bm{u}}[\Theta^i]
\end{align}
where $ \int \rho \theta = $. Taking limits takes us back to what was derived in the text. 

Hmm discretize differently

\begin{align}
    \partial_t \bm{\theta} + Q[\bm{u}, \bm{\theta} ] &= D[ \bm{\theta} ] + \bm{s}
\end{align}
with multi-linear operator $Q$ and linear operator $D$. 

For the variance equation one sees that the co-variance is necessary. Thus we need a 6-D pde for a 3D advection diffusion equation. This may not be a big deal if only nearest neighbors are correlated, as one would expect far away from boundaries. This would imply that the structure of the 6D pde can be reduced to coupled 3D pde's where only the nearest neighbors are required. 

\subsection{Linear Algebraic point of view}
Perhaps instead rewrite things in terms of complements and such
\begin{align}
    \begin{bmatrix}
    a & \bm{w}^T \\
    \bm{v} & L 
    \end{bmatrix}
    \begin{bmatrix}
    \langle \theta \rangle \\
    \bm{\theta}'
    \end{bmatrix}
    = 
    \begin{bmatrix}
    s(\bm{x}) \\
    \bm{0}
    \end{bmatrix}
\end{align}
So that the equation for $\langle \theta \rangle$ is 
\begin{align}
    a \avg{\theta} + \bm{w}^T L^{-1} \bm{v} \avg{\theta } = s(\bm{x})
\end{align}
Then the goal would be to just write the pieces, $\bm{w}^T$, $L^{-1}$, $\bm{v}$.


For example, in the two state system we would have 
\begin{align}
\begin{bmatrix}
-\Delta & \nabla \cdot( \bm{u} \cdot ) \\
\bm{u} \cdot \nabla  & \gamma - \Delta 
\end{bmatrix}
\begin{bmatrix}
\langle \theta \rangle \\
\varphi 
\end{bmatrix} 
= 
\begin{bmatrix}
s(\bm{x}) \\
0 
\end{bmatrix}
\end{align}
Thus $L = \gamma - \Delta $, $\bm{w}^T = \nabla \cdot( \bm{u} \cdot )$, and $\bm{v} = \bm{u} \cdot \nabla $. Since $\bm{u} \cdot \nabla = \nabla \cdot \left( \bm{u} \cdot \right)$ for a incompressible flow field.

and in the three state system 

\begin{align}
\begin{bmatrix}
-\Delta & \nabla \cdot( \bm{u} \cdot ) & 0 \\
\frac{1}{2}\bm{u} \cdot \nabla  & \gamma - \Delta  & \frac{1}{2}\bm{u} \cdot \nabla  \\
0                               & \bm{u} \cdot \nabla & - \Delta + 2 \gamma 
\end{bmatrix}
\begin{bmatrix}
\varphi_1 \\
\varphi_2 \\
\varphi_3
\end{bmatrix} 
= 
\begin{bmatrix}
s(\bm{x}) \\
0  \\
0
\end{bmatrix}
\end{align}
Here 
\begin{align}
    L = \begin{bmatrix}
 \gamma - \Delta  & \frac{1}{2}\bm{u} \cdot \nabla  \\
 \bm{u} \cdot \nabla & - \Delta + 2 \gamma 
    \end{bmatrix}
    \text{ , } 
\bm{v} = 
\begin{bmatrix}
\frac{1}{2}\bm{u} \cdot \nabla  \\
0 
\end{bmatrix}
\text{ , and } 
\bm{w}^T = 
\begin{bmatrix}
\nabla \cdot( \bm{u} \cdot ) & 0 
\end{bmatrix}
\end{align}
we only need top component of $L^{-1} \bm{v}$ . The inverse of two by two block matrix 
\begin{align}
R = 
    \begin{bmatrix}
    A & B \\
    C & D
    \end{bmatrix}
\end{align}
is 
\begin{align}
R^{-1} = 
    \begin{bmatrix}
    (A- B D^{-1} C)^{-1} & - (A- B D^{-1} C)^{-1} B D^{-1} \\
    - D^{-1}C (A- B D^{-1} C)^{-1} & (D- C A^{-1} B)^{-1}
    \end{bmatrix}
\end{align}
In the case of the three state system we only need the top left corner. 
\begin{align}
  L^{-1} = 
  \begin{bmatrix}
  \left(\gamma - \Delta - \frac{1}{2} \bm{u} \cdot \nabla (2 \gamma - \Delta)^{-1} \bm{u} \cdot \nabla \right)^{-1} & * \\
  * & * 
  \end{bmatrix}
\end{align}
In general the $\bm{v}$ will be some weighted sum of the transition states dotted into nabla, and the $\bm{w}$ is similar. 

Numerically we can construct the block operators and invert them. Thus for a more complex coupled systems this may become necessary

\subsection{Alternative Derivation ?}
\begin{align}
\partial_t \theta + \nabla \cdot ( \bm{u} \theta - \kappa \nabla \theta) &= s
\partial_t \langle \theta \rangle_m + \nabla \cdot (\langle \bm{u} \theta \rangle_m - \kappa \nabla \langle \theta \rangle_m ) &=  s \\
P_m \partial_t \langle \theta \rangle_m + \nabla \cdot P_m (\langle \bm{u} \theta \rangle_m - \kappa \nabla \langle \theta P_m \rangle_m ) &=  sP_m \\
\partial_t(P_m \langle \theta \rangle_m) - \partial_t P_m \langle \theta \rangle_m  + \nabla \cdot P_m (\langle \bm{u} \theta \rangle_m - \kappa \nabla \langle \theta P_m \rangle_m ) &=  sP_m  \\
\partial_t(P_m \langle \theta \rangle_m) - Q_{mn} P_n \langle \theta \rangle_m  + \nabla \cdot P_m (\langle \bm{u} \theta \rangle_m - \kappa \nabla \langle \theta P_m \rangle_m ) &=  sP_m  \\
\end{align}
no commutation: $\partial_t \langle \theta \rangle_m  \neq \langle \partial_t \theta \rangle_m$, means that this simpler derivation is somewhat not great.

Apparently the implicication is that 
\begin{align}
   \mathbb{P}[\bm{u}_\omega(\bm{x}, t) = \bm{u}_m(\bm{x})] \langle \partial_t \theta_\omega \rangle_{\bm{u}_\omega(\bm{x}, t) = \bm{u}_m(\bm{x})} &= \partial_t \left( \mathbb{P}[\bm{u}_\omega(\bm{x}, t) = \bm{u}_m(\bm{x})] \langle \theta_\omega \rangle_{\bm{u}_\omega(\bm{x}, t) = \bm{u}_m(\bm{x})}  \right) \\
   &-  \sum_{n} \mathcal{Q}_{mn} \left( \mathbb{P}[\bm{u}_\omega(\bm{x}, t) = \bm{u}_n(\bm{x})] \langle \theta_\omega \rangle_{\bm{u}_\omega(\bm{x}, t) = \bm{u}_n(\bm{x})}  \right)
\end{align}

abbreviating
\begin{align}
   P_m \langle \partial_t \theta \rangle_{m} &= \partial_t \left( P_m  \langle \theta \rangle_{m}  \right) -  \sum_{n} \mathcal{Q}_{mn} \left( P_n \langle \theta \rangle_{n}  \right)
   \\
   &\Leftrightarrow 
   \\
   \langle \theta \rangle_m \partial_t P_m &= \sum_n \mathcal{Q}_{mn} P_n \langle \theta \rangle_n + P_m \left( \partial_t \langle \theta \rangle_m -  \langle \partial_t \theta \rangle_m \right)
   \\
   \langle \theta \rangle_m \sum_{n} \mathcal{Q}_{mn} P_n &= \sum_n \mathcal{Q}_{mn} P_n \langle \theta \rangle_n + P_m \left( \partial_t \langle \theta \rangle_m -  \langle \partial_t \theta \rangle_m \right)
   \\
   0 &= \sum_n \mathcal{Q}_{mn} P_n (\langle \theta \rangle_n - \langle \theta \rangle_m) + P_m \left( \partial_t \langle \theta \rangle_m -  \langle \partial_t \theta \rangle_m \right)
\end{align}

==> Sections/old_conclusions.tex <==
\section{Conclusions}
\label{conclusions}

We focused on computing turbulent-fluxes of a statistically steady state. With regards to modeling this may suffice to get the statistical dynamics correct depending on the level of coarse graining. See Neeraja et al. for an example that does this. 

If one considers a hiearchy of coarse graining procedures then the role of nonlocality becomes more prominent. For example, in the first level of coarse graining, perhaps a local closure suffices. Okay great we use it. Now let's go to the next level of the hiearchy. Now the effective diffusivity that we obtained in the previous step is quite high. We go to the next level of coarse graining. Our large diffusivity will now contribute to an effective nonlocal turbulent flux closure for the larger scale flow that we are considering. Thus the expectation is that non-locality becomes prominent as multiscale features are considered. 

Here we have outlined a method where we assume that the flow fields and transition probabilities are given a priori. It would be interesting to carry out such an analysis for turbulent flows. The idea would be to estimate coherent structures and their transition probabilities so as to create a model that conforms to one amenable to the analysis prescribed here. If the mean statistics of a passive tracer with such a model is reproduces that of a passive tracer in a turbulent field, then one can claim that the underlying structures organize the flow. 

A harder task is then to estimate a priori, without running simulations, a set of flow structures and transition probabilities. A finite volume discretization of the Hopf equation would provide a guide, but one would need to apriori select points in function space to interpolate around. Perhaps a hieararchical approach based on modes of a numerical method would work. Another option is to directly discretize the Fokker-Planck operator in terms of infinite dimensional analogues of hermite expansions. Again a spectral decomposition seems useful. 

Large scale slowly moving coherent structures add significant nonlocality

==> Sections/old_example.tex <==

\subsection{Mean-zero Two-State System}

Consider a one-dimensional incompressible flow field that transitions between a $u_1 = +U$ velocity and a $u_2 = -U$ velocity with a transition probability matrix given by 
\begin{align}
    [T]_{mn} &= \gamma
    \begin{bmatrix}
        -1/2 & 1/2 \\
        1/2 & -1/2
    \end{bmatrix}
\end{align}
The passive tracer equation is 
\begin{align}
    \partial_t \theta + u(t) \partial_x \theta &= \partial_{xx} \theta + s(x).
\end{align}
We withhold specifying the domain and boundary conditions for now. In order for there to be a statistically steady state there need to be compatibility conditions in the source terms, boundary conditions, and domain. For example, for a periodic domain the source term must also have mean zero.

As given by the general theory the equation for the mean statistics is 
\begin{align}
\partial_t P_{1} &= \gamma (- P_{1} + P_{2}) /2 
\\
\partial_t P_{2} &= \gamma (P_{1} - P_{2}) /2 
\\
\partial_t \Theta_1 + U \partial_x \Theta_1 &= \partial_{xx} \Theta_1 + s(x) P_{1} + \gamma (-\Theta_1 + \Theta_2)/2 \\
\partial_t \Theta_2 - U \partial_x \Theta_2 &= \partial_{xx} \Theta_2 + s(x) P_{2} + \gamma (\Theta_1 - \Theta_2)/2
\end{align}
Focusing on the statistically steady state yields $P_1 = P_2 = 1/2$ and 
\begin{align}
\label{mean_equation_2_state}
U \partial_x \Theta_1 &= \partial_{xx} \Theta_1 + s(x)/2 +  \gamma (-\Theta_1 + \Theta_2)/2 
\\
- U \partial_x \Theta_2 &= \partial_{xx} \Theta_2 + s(x)/2 + \gamma (\Theta_1 - \Theta_2)/2
\end{align}
We change variables to $\avg{ \theta } = (\Theta_1 + \Theta_2)/2$ and $\varphi = (\Theta_1 - \Theta_2)/2$ so that \eref{mean_equation_2_state} becomes 
\begin{align}
\label{mean_equation_2_state}
\partial_x (U \varphi) &= \partial_{xx} \langle \theta \rangle  + s(x)
\\
\partial_x \left( U \langle \theta \rangle \right)  &= \partial_{xx} \varphi - \gamma \varphi
\end{align}
Introducing the Green's function $(-\gamma  + \partial_{xx})^{-1}$ we solve for $\varphi$ in terms of the gradients of $\langle \theta \rangle$ and 
\begin{align}
\label{mean_equation_2_state}
\partial_x (U( -\gamma  +\partial_{xx})^{-1} \left( U \partial_x \avg{\theta} \right) ) &= \partial_{xx} \langle \theta \rangle  + s(x)
\end{align}

We recognize the turbulent-flux term,
\begin{align}
    \langle \bm{u}' c' \rangle = U(-\gamma + \partial_{xx})^{-1} \left( U \partial_x \avg{\theta} \right)
\end{align}
and the kernel operator
\begin{align}
\int dx' \mathcal{K}(x | x')  = U (-\gamma + \partial_{xx})^{-1} U
\end{align}
We see that mixing in this model is tied to the diffusive mechanism. At small scales transport becomes ineffecitive due to the presence of diffusion. The tracer diffusives before advection has a change to transport it.  The smaller the length scale the stronger the dominance of diffusion. 

The solution for the mean is then 
\begin{align}
\langle \theta \rangle &= (-\partial_{xx} + U \partial_x (-\gamma  + \partial_{xx})^{-1}\left(U \partial_x \right))^{-1} s(x)
\end{align}

Assuming a fourier decomposition 
\begin{align}
\langle \theta \rangle_k &= \frac{s_k}{k^2 + U^2 k^2 / (\gamma + k^2) }
\end{align}

It is also possible to solve this problem by first decomposing the stochastic PDE into Fourier modes, leading to an infinite set of uncouple ode's. Writing down the Fokker-Planck equation for each fourier mode. Writing down the mean equations from the Fokker-Planck equations, solving for the turbulent-fluxes and mean mode, and then synthesizing back. At the end of the tedium one gets back to the above solution. 

The calculations above may be repeated for the case where one is transition between and incompressible flow field $\pm \bm{u}(\bm{x})$ with a dissipation mechanism given by a linear operator $\bm{D}$ that is, if 
\begin{align}
    \partial_t \theta + \bm{u} \cdot \nabla \theta &= \bm{D}[\theta] +  s(\bm{x})
\end{align}
then 
\begin{align}
\langle \bm{u}' \theta' \rangle = \bm{u}(-\gamma + \bm{D})^{-1} \left( \bm{u}\cdot \nabla \langle \theta \rangle \right)
\end{align}


\subsection{Continuous in Time in Theory}
Decompose $\bm{u}_\omega = a_\omega(t)\bm{u}(\bm{x})$ for a fixed flow structure $\bm{u}(\bm{x})$.
The master equation for the stochastic partial differential equation
\begin{align}
    \partial_t \theta_{\omega} +  \nabla \cdot \left( a_\omega(t)\bm{u}(\bm{x})  \theta_{\omega} - \kappa \nabla \theta_\omega \right) &=  s_{\omega}(\bm{x} ) 
    \\
    d a_\omega &= f(a) dt + \sigma dW_\omega
\end{align}
is
\begin{align}
\label{hopfs_eqn_2}
\partial_t \rho &= -\int d\mathbf{x} \frac{\delta}{\delta \theta }\left( \left[  - \nabla \cdot \left( a \mathbf{u} \theta - \kappa \nabla \theta \right)  + s \right] \rho \right) - \partial_{a} \left( f(a) \rho -  \sigma^2/2 \partial_{a} \rho \right)
\end{align}
The equation for the mean then becomes
\begin{align}
    \partial_t P &=  - \partial_{a} \left( f(a) \rho -  \sigma^2/2 \partial_{a} \rho \right) 
    \\
    \partial_t \Theta + \nabla \cdot \left( a \bm{u} \Theta - \kappa \nabla \Theta \right)  &= P(a) s(x) - \partial_{a} \left( f(a) \Theta -  \sigma^2/2 \partial_{a} \Theta \right)
\end{align}
We see that, depending on the number of stochastic variables necessary to describe the evolution of the stochastic flow field $\bm{u}$, we have to solve an $n+n_{\bm{u}}$ dimensional PDE for the mean statistics of $\theta$.

We can also choose $\bm{u}_{\bm{\omega}} = \sum_n {a_n}_{\omega}(t)\bm{u}_n(\bm{x}) $ for $n$ independent flow structures and ${a_{n}}_{\omega}$ stochastic processes and get similar equations. 


\subsection{3 State System}

Consider a three state sytem $(u_1 , u_2, u_3) = (-\bm{u}(\bm{x}), 0, \bm{u}(\bm{x}) )$ with transition probability
\begin{align}
T_{nm} &= \gamma 
\begin{bmatrix}
-1.0 & 0.5 & 0.0 \\
1.0 & -1.0 & 1.0 \\
0.0 & 0.5 & -1.0
\end{bmatrix}
\end{align}

The equations to solve for are
\begin{align}
    \partial_t P_m &= \sum_{n} T_{mn} P_n \\
    \partial_t \Theta_m + u_m \cdot \nabla \Theta_m &= D \Theta_m + P_m s(\bm{x} ) + \sum_{n} T_{mn} \Theta_n
\end{align}
where $D$ is a negative semi-definite operator. 
Solving for the statistically steady state for $P_n$ yields 
\begin{align}
    P = \begin{bmatrix}
    1/4 & 
    1/2 &
    1/4
    \end{bmatrix}
\end{align}
We recombine $\Theta_m$ in terms of the left eigenvector (Koopman modes / EOF) of the transition matrix $T_{mn}$, which are
\begin{align}
v^1 &= \begin{bmatrix}
1 \\ 
1 \\
1
\end{bmatrix}
\text{ , }
v^2 = 
\begin{bmatrix}
-1 \\
0 \\
1
\end{bmatrix}
\text{ and, }
v^3 = 
\begin{bmatrix}
1 \\
-1 \\
1
\end{bmatrix}
\end{align}
with eigenvalues $(\lambda^1 , \lambda^2, \lambda^3) = (0, -\gamma, -2\gamma)$. We recombine $\Theta_n$ according to the left eigenvectors, i.e.
\begin{align}
    \varphi_1 &= \Theta_1 + \Theta_2 + \Theta_3 \\
    \varphi_2 &= -\Theta_1 + \Theta_3 \\
    \varphi_3 &= \Theta_1 - \Theta_2 + \Theta_3
\end{align}
so that the system of equations becomes
\begin{align}
\bm{u} \cdot \nabla  \left( \varphi_2 \right) &= D \varphi_1 + s(\bm{x})
\\
\frac{1}{2}\bm{u} \cdot \nabla  \left( \varphi_1 + \varphi_3 \right) &= D \varphi_2 - \gamma \varphi_2 
\\
\bm{u} \cdot \nabla  \left( \varphi_2 \right) &= D \varphi_3 - 2 \gamma \varphi_3
\end{align}
we observe that $\varphi_1 = \langle \theta \rangle$. Solving for $\varphi_3$ in terms of $\varphi_2$ yields
\begin{align}
\varphi_3 &= (D- 2 \gamma)^{-1}\left( \bm{u} \cdot \nabla  \left( \varphi_2 \right) \right)
\end{align}
We rearrange the $\varphi_2$ equation 
\begin{align}
    \frac{1}{2}\bm{u} \cdot \nabla  \left( \varphi_1 \right) &= D \varphi_2 - \gamma \varphi_2  - \frac{1}{2} \bm{u} \cdot \nabla \left( \varphi_3 \right) \\
    &= D \varphi_2 - \gamma \varphi_2  - \frac{1}{2} \bm{u} \cdot \nabla \left( (D- 2 \gamma)^{-1}\left( \bm{u} \cdot \nabla  \left( \varphi_2 \right) \right) \right)
\end{align}
Solving for $\varphi_2$ in terms of $\varphi_1$ yields 
\begin{align}
    \varphi_2  = \left[ D  - \gamma   - \frac{1}{2} \bm{u} \cdot \nabla \left( (D- 2 \gamma)^{-1}\left( \bm{u} \cdot \nabla  \right) \right) \right]^{-1} \left[ \frac{1}{2}\bm{u} \cdot \nabla  \left( \varphi_1 \right) \right]
\end{align}
To get the turbulent flux 
\begin{align}
    \langle \bm{u}' \theta' \rangle &= \bm{u} \varphi_2 = \bm{u}  \left[ D  - \gamma   - \frac{1}{2} \bm{u} \cdot \nabla \left( (D- 2 \gamma)^{-1}\left( \bm{u} \cdot \nabla  \right) \right) \right]^{-1} \left[ \frac{1}{2}\bm{u} \cdot \nabla  \left( \langle \theta \rangle \right) \right]
\end{align}
which means that the kernel operator is 
\begin{align}
    \int d \bm{x} \mathcal{K}(\bm{x} | \bm{x}' ) = \bm{u}  \left[ D  - \gamma   - \frac{1}{2} \bm{u} \cdot \nabla \left( (D- 2 \gamma)^{-1}\left( \bm{u} \cdot \nabla  \right) \right) \right]^{-1} \frac{1}{2} \bm{u}^T
\end{align}


This section outlined the general procedure. Let $v_m^i$ denote the $i'th$ component of the left eigenvectors of the transition matrix. Taking the inner product of the $i'th$ vector with the equation 
\begin{align}
    \partial_t \Theta_m + \bm{u}_m \cdot \nabla \Theta_m &= D \Theta_m + P_m \bm{s}(\bm{x}) + \sum_n T_{m n } \Theta_n
\end{align}
to get 

\begin{align}
    \partial_t \sum_{m} v^i_m \Theta_m + \sum_{m} v^i_m  \bm{u}_m \cdot \nabla \Theta_m &= D \sum_{m} v^i_m \Theta_m + \sum_{m} v^i_m P_m \bm{s}(\bm{x}) + \sum_{m} v^i_m \sum_n T_{m n } \Theta_n
\end{align}
and use the fact that the $P_m$ will be the zero'th mode (right eigenvector corresponding to the eigenvalue zero) in a statistically steady state 
\begin{align}
    \partial_t \varphi^i + \sum_{m} v^i_m  \bm{u}_m \cdot \nabla \Theta_m &= D \varphi^i  + \delta_{i1} \bm{s}(\bm{x}) + \lambda^i \varphi^i
\end{align}
where $\varphi^i = \sum_{m} \varphi^i_m \Theta_m$. The term $\sum_{m} v^i_m  \bm{u}_m \cdot \nabla \Theta_m$ must be rewritten into something involving gradients of $\varphi^i$ and some exceptional flow fields $\bm{u}^i$. 

The generalization to infinite dimensional transition matrices is similar. One needs to project the equations on to the basis of the eigenvectors of the Fokker-Planck operator. The left eigenvectors serve as a convenient way of projecting. In order to make a correspondence to the average field the projection must be normalized. Letting $i = 1$, the ground state, we can see the correspondence with the average. Just need to change basis on the advection thing. A similarity transformation on the operator $V U V^{-1} = A$. Where $U = Diagonal([\bm{u}_1 \bm{u}_2 ... \bm{u}_n])$. The $V U V^{-1}$ is a natural recombination of the states. 

For example for the three state system
\begin{align}
U = u
    \begin{bmatrix}
    -1 & 0 &0 \\
    0 & 0 & 0 \\
    0 & 0 & 1
    \end{bmatrix}
    W = 
    \begin{bmatrix}
    1 & 1 & 1 \\
    1 & 0 & -1 \\
    1 & -1 & 1
    \end{bmatrix}
    W^{-1}  = \frac{1}{4}
        \begin{bmatrix}
    1 & 2 & 1 \\
    2 & 0 & -2 \\
    1 & -2 & 1
    \end{bmatrix}
    W U W^{-1}
    = 
    -
    \begin{bmatrix}
    0 &  1 & 0 \\
    1/2 & 0 & 1/2 \\
    0 & 1 & 0 
    \end{bmatrix}
\end{align}
In other words we want to express the advection operator in the transition matrix basis. In the ``ensemble member" basis it is diagonal. 

\subsection{Four State Phase Shift}
We work in the domain $x \in [0, 2 \pi)$ and $z \in [-1, 1]$ with transition stream functions
\begin{align}
    \psi_1 &= \sin(x) \cos\left(\frac{\pi}{2}z\right) \text{, }
    \psi_2 = \cos(x) \cos\left(\frac{\pi}{2}z\right) \text{, } 
    \\
    \psi_3 &= - \sin(x) \cos\left(\frac{\pi}{2}z\right) \text{, and }
    \psi_4 = - \cos(x) \cos\left(\frac{\pi}{2}z\right),
\end{align}
with transition matrix 
\begin{align}
    T &= \gamma 
    \begin{bmatrix}
    -1 & 1/2 & 0 & 1/2 \\
    1/2 & -1 & 1/2 & 0 \\
    0 & 1/2 & -1 & 1/2 \\
    1/2 & 0 & 1/2 & -1
    \end{bmatrix}
    + 
    \omega 
    \begin{bmatrix}
    0 & 1/2 & 0 & -1/2 \\
    -1/2 & 0 & 1/2 & 0 \\
    0 & -1/2 & 0 & 1/2 \\
    1/2 & 0 & -1/2 & 0
    \end{bmatrix}
\end{align}
which has eigenvalues $0, -\gamma - \omega \iota, -\gamma + \omega \iota, -2 \gamma$.
Eigenvectors
\begin{align}
V = 
\begin{bmatrix}
 1.0  &  1.0   & 1.0  &  1.0 \\ 
 1.0  &  - \iota & \iota   & -1.0 \\
 1.0  & -1.0   & -1.0  &  1.0 \\
 1.0  &  \iota  & -\iota  & -1.0 
\end{bmatrix}
\end{align}
To avoid imaginary stuff just take combinations of the form $(v^2 + v^3)/2$ and $(v^2 - v^3)/(2 \iota)$. This linear combinations will be orthogonal to everything else  since $v^2$ and $v^3$ are orthogonal.
Use different similarity transformation to avoid introducing imaginary things at the cost of explicit coupling. The $S^{-1}$ projects onto the basis vectors defined by the columns of $S$,
\begin{align}
S^{-1}  = 
\begin{bmatrix}
 1.0  &  1.0   & 1.0  &  1.0 \\ 
 1.0  &  0.0   & -1.0  & 0.0 \\
 0.0  & 1.0   & 0.0  &  -1.0 \\
 1.0  &  -1.0 & 1.0  & -1.0 
\end{bmatrix}
\text{ and }
S = 
\begin{bmatrix}
 1/4  &  1/2  & 0     &  1/4 \\ 
 1/4  &  0    & 1/2   & -1/4 \\
 1/4  & -1/2  & 0     &  1/4 \\
 1/4  &  0    & -1/2  & -1/4 
\end{bmatrix}
\end{align}

Perhaps write system of equations this way
\begin{align}
\bm{u}_1 \cdot \nabla \Theta_1 
 &= D\Theta_1 + s(x,z)/4 - \gamma \Theta_1 + \Theta_2 (\gamma + \omega)/2  + \Theta_4 (\gamma - \omega)/2 
 \\
 \bm{u}_2 \cdot \nabla \Theta_2 
 &= D\Theta_2 + s(x,z)/4 - \gamma \Theta_2 + \Theta_3 (\gamma + \omega)/2  + \Theta_1 (\gamma - \omega)/2 
 \\
 \bm{u}_3 \cdot \nabla \Theta_3 
 &= D\Theta_3 + s(x,z)/4 - \gamma \Theta_3 + \Theta_4 (\gamma + \omega)/2  + \Theta_2 (\gamma - \omega)/2 
 \\
 \bm{u}_4 \cdot \nabla \Theta_4 
 &= D\Theta_4 + s(x,z)/4 - \gamma \Theta_4 + \Theta_1 (\gamma + \omega)/2  + \Theta_3 (\gamma - \omega)/2 
\end{align}

With this transition matrix in place our statistically steady system of equations becomes
\begin{align}
\begin{bmatrix}
\bm{u}_1 \cdot \nabla - D  + \gamma  & -(\gamma + \omega)/2  & 0  & -(\gamma - \omega)/2 
\\
 -(\gamma - \omega)/2  & \bm{u}_2 \cdot \nabla - D  + \gamma & -(\gamma + \omega)/2 & 0 
\\
0 &  -(\gamma - \omega)/2  & \bm{u}_3 \cdot \nabla - D  + \gamma & -(\gamma + \omega)/2
\\
-(\gamma + \omega)/2 & 0 &  -(\gamma - \omega)/2  & \bm{u}_4 \cdot \nabla - D + \gamma 
\end{bmatrix}
\begin{bmatrix}
\Theta_1 \\
\Theta_2 \\
\Theta_3 \\
\Theta_4
\end{bmatrix}
&=
\begin{bmatrix}
s(x,z)/4 \\
s(x,z)/4 \\
s(x,z)/4 \\
s(x,z)/4 \\
\end{bmatrix}
\end{align}


The first and last column diagonalize the operator but the middle two do not. Letting $U = \text{Diagonal}(u_1, u_2, u_3, u_4)$ the transformation yields
\begin{align}
S U S^{-1} = 
    \begin{bmatrix}
    \frac{u_1 + u_2 + u_3 + u_4}{4} & \frac{u_1 - u_3}{2} & \frac{u_2 - u_4}{2} & \frac{u_1 - u_2 + u_3 - u_4}{4}
    \\
    \frac{u_1 - u_3}{4} & \frac{u_1 + u_3}{2} & 0 & \frac{u_1 - u_3}{4}
    \\
    \frac{u_2 - u_4}{4} & 0 & \frac{u_2 + u_4}{4} & -\frac{u_2 - u_4}{4}
    \\
    \frac{u_1 - u_2 + u_3 - u_4 }{4}& \frac{u_1 - u_3}{2} & \frac{u_2 - u_4}{2} & \frac{u_1 + u_2 + u_3 + u_4}{4}
    \end{bmatrix}
\end{align}
and the transition matrix part (since we no longer have eigenvectors)
\begin{align}
S T S^{-1} = 
    \begin{bmatrix}
    0 & 0 &0 & 0 \\
    0 & -\gamma & \omega & 0 \\
    0 & -\omega & -\gamma & 0 \\
    0 & 0 & 0 & -2 \gamma
    \end{bmatrix}
\end{align}
The rest of the structure is okay. On the diagonal we have the dissipation structure. The source term is still on the top index. But it seems like everything is coupled together now. The phase information is somewhat kept intact in the transition matrix.

We make the change of variables
\begin{align}
 \begin{bmatrix}
 1.0  &  1.0   & 1.0  &  1.0 \\ 
 1.0  &  0.0   & -1.0  & 0.0 \\
 0.0  & 1.0   & 0.0  &  -1.0 \\
 1.0  &  -1.0 & 1.0  & -1.0 
\end{bmatrix}
\begin{bmatrix}
\Theta_1 \\
\Theta_2 \\
\Theta_3 \\
\Theta_4
\end{bmatrix}
= 
\begin{bmatrix}
\langle \theta \rangle \\
\varphi_1 \\
\varphi_2 \\
\varphi_3
\end{bmatrix}
\end{align}

using $\bm{u}_1 = - \bm{u}_3$ and $\bm{u}_2 = - \bm{u}_4$.
The system of equations becomes
\begin{align}
\begin{bmatrix}
- D & \nabla \cdot \left( \bm{u}_1 \cdot \right) & \nabla \cdot \left( \bm{u}_2 \cdot \right)  & 0 
\\
\frac{1}{2}\bm{u}_1 \cdot \nabla & \gamma - D & -\omega & \frac{1}{2}\bm{u}_1 \cdot \nabla  
\\
\frac{1}{2}\bm{u}_2 \cdot \nabla  & \omega  & \gamma - D & - \frac{1}{2} \bm{u}_2 \cdot \nabla  
\\
0    & \bm{u}_1 \cdot \nabla  & - \bm{u}_2 \cdot \nabla  & 2\gamma - D
\end{bmatrix}
\begin{bmatrix}
\langle \theta \rangle \\
\varphi_1 \\
\varphi_2 \\
\varphi_3
\end{bmatrix}
&=
\begin{bmatrix}
s(\bm{x}) \\
0 \\
0 \\
0 \\
\end{bmatrix}
\end{align}

Perhaps an insight is the following. Once something is in a statistically steady state there are more ways to combine ensemble members than just a simple average and still get a statistically steady object. Each conditional mean is also in a statistically steady state. 

Specifically we may compare to local turbulent diffusivity estimates from Glenn et al. For a flow field with the  structure
\begin{align}
\psi(x,z,t) = a(t) \sin(k  x) \sin(\ell z)
\end{align}
The local turbulent-diffusivity has the structure
\begin{align}
    K_{11} &= \kappa \cos^2 ( \ell z) \text{, }  K_{22} = \kappa \frac{k^2}{\ell^2} \sin^2(\ell y) \\
    K_{12} &= \kappa \frac{k}{\ell} \tilde{f} \sin(\ell y) \cos(\ell y) = - K_{21}
\end{align}
where the diffusivity amplitude $\kappa$ and dimensionless frequency $\tilde{f}$ depend on the flow statistics determined by $a(t)$. We emphasize that the above only applies when neglecting diffusive and nonlocal effects.

We obtain a local diffusivity estimate by treating $D=0$ and $\varphi_3 = 0$ (or perhaps more accurately neglective diffusivity and performing an expansion in terms of the amplitude of the velocity and neglecting contributions that are more than quadratic). The local diffusivity tensor is

\begin{align}
\bm{K} = 
    \frac{1}{2( \gamma^2 + \omega^2)}
    \begin{bmatrix}
    \bm{u}^1 & \bm{u}^2 
    \end{bmatrix}
    \begin{bmatrix}
    \gamma & \omega \\
    -\omega & \gamma 
    \end{bmatrix}
        \begin{bmatrix}
    \bm{u}^1 \\
    \bm{u}^2 
    \end{bmatrix}
\end{align}

where 
\begin{align}
    \bm{u}_i &= \partial_z \psi_i \hat{x} + (-\partial_x \psi_i ) \hat{z}
\end{align}
which implies 
\begin{align}
    \bm{u}_1 &= -\frac{\pi}{2} \sin(x) \sin \left(\frac{\pi}{2} z \right) \hat{x} - \cos(x) \cos \left( \frac{\pi}{2} z \right) \hat{z} 
    \\
    \bm{u}_2 &= -\frac{\pi}{2} \cos(x) \sin \left(\frac{\pi}{2} z \right) \hat{x} + \sin(x) \cos \left( \frac{\pi}{2} z \right) \hat{z} 
\end{align}
The local estimates are
\begin{align}
K^{xx} &=  
    \begin{bmatrix}
    \frac{\pi}{2} \sin(x) \sin \left(\frac{\pi}{2} z \right) & \frac{\pi}{2} \cos(x) \sin \left(\frac{\pi}{2} z \right) 
    \end{bmatrix}
    \begin{bmatrix}
    \frac{\gamma}{2( \gamma^2 + \omega^2)} & \frac{\omega}{2( \gamma^2 + \omega^2)} \\
    -\frac{\omega}{2( \gamma^2 + \omega^2)} & \frac{\gamma}{2( \gamma^2 + \omega^2)}
    \end{bmatrix}
        \begin{bmatrix}
    \frac{\pi}{2} \sin(x) \sin \left(\frac{\pi}{2} z \right) \\
    \frac{\pi}{2} \cos(x) \sin \left(\frac{\pi}{2} z \right)
    \end{bmatrix}
    \\
    &=
    \frac{\gamma \pi^2}{8(\gamma^2 + \omega^2)} \sin^2 \left(\frac{\pi}{2} z \right)
    \\
K^{xz} &=  
    \begin{bmatrix}
    -\frac{\pi}{2} \sin(x) \sin \left(\frac{\pi}{2} z \right) & -\frac{\pi}{2} \cos(x) \sin \left(\frac{\pi}{2} z \right) 
    \end{bmatrix}
    \begin{bmatrix}
    \frac{\gamma}{2( \gamma^2 + \omega^2)} & \frac{\omega}{2( \gamma^2 + \omega^2)} \\
    -\frac{\omega}{2( \gamma^2 + \omega^2)} & \frac{\gamma}{2( \gamma^2 + \omega^2)}
    \end{bmatrix}
        \begin{bmatrix}
   -\cos(x) \cos \left( \frac{\pi}{2} z \right) \\
    \sin(x) \cos \left( \frac{\pi}{2} z \right)
    \end{bmatrix}
    \\
    &=
    \frac{\omega \pi}{4(\gamma^2 + \omega^2)} 
    \sin \left( \frac{\pi}{2} z \right) \cos \left( \frac{\pi}{2} z \right) 
    \\
K^{zx} &= - K^{z x} =  
    -\frac{\omega \pi}{4(\gamma^2 + \omega^2)} 
    \sin \left( \frac{\pi}{2} z \right) \cos \left( \frac{\pi}{2} z \right)
    \\
K^{zz} &=    
    \begin{bmatrix}
     -\cos(x) \cos \left(\frac{\pi}{2} z \right) &  \sin(x) \cos \left(\frac{\pi}{2} z \right) 
    \end{bmatrix}
    \begin{bmatrix}
    \frac{\gamma}{2( \gamma^2 + \omega^2)} & \frac{\omega}{2( \gamma^2 + \omega^2)} \\
    -\frac{\omega}{2( \gamma^2 + \omega^2)} & \frac{\gamma}{2( \gamma^2 + \omega^2)}
    \end{bmatrix}
    \begin{bmatrix}
    -\cos(x) \cos \left(\frac{\pi}{2} z \right) \\
    \sin(x) \cos \left(\frac{\pi}{2} z \right) 
    \end{bmatrix}
    \\
    &=
    \frac{\gamma }{2(\gamma^2 + \omega^2)} \cos^2 \left(\frac{\pi}{2} z \right)
\end{align}

In general the connection to Taylor's hypothesis would be to take the inverse of the transition matrix and let it act on the statistically determined flow fields while neglecting diffusive and additional advective contributions. This will basically involve the first row and column of the $SUS^{-1}$ matrix and the lower block of the $STS^{-1}$ matrix. Perhaps writing it as the inverse orthogonal projection? In some sense it doesn't really matter what the similarity transformation is, what matters is that the top row must by the one matrix and first column must be $P_m$. Thus as long as the other vectors are orthogonal we are okay. 

\begin{figure}
  \centerline{\includegraphics[width=1\textwidth]{Figures/local_case.png}}% Images in 100% size
  \caption{Local diffusivity estimate in red and Numerically computed diffusivity estimate blue dots. This is a case where the local diffusivity assumption is good $\gamma$ is large and the diffusivity is zero and the flow amplitude is order one. The y-axis is depth and the x-axis is the diffusivity amplitude. Here $\gamma = \omega = 100$ and $\kappa = 1/100$. The results are roughly independent of $\kappa$ in the limit $\kappa \rightarrow 0$.}
\label{fig:local_local_diffusivity}
\end{figure}

\begin{figure}
  \centerline{\includegraphics[width=1\textwidth]{Figures/nonlocal_case.png}}% Images in 100% size
  \caption{Local diffusivity estimate in red and Numerically computed diffusivity estimate blue dots. This is a case where the local diffusivity assumption is bad $\gamma$  and the diffusivity and the flow amplitude are all order one.  The y-axis is depth and the x-axis is the diffusivity amplitude. Here $\gamma = \omega = 1$ and $\kappa = 1$.}
\label{fig:nonlocal_local_diffusivity}
\end{figure}


\begin{figure}
  \centerline{\includegraphics[width=1\textwidth]{Figures/local_kernel.png}}% Images in 100% size
  \caption{A representation of the full diffusivity kernel corresponding to the case in Figure \ref{fig:local_local_diffusivity}. If the diffusivity was indeed local then each of the form matrices would only have a diagonal component. The x-y coordinate axis have been collapsed to a single index, hence the banded structure of the output. Thus the rows are the "output" axis corresponding to the $(x,z)$ of $K(x,z|x',z')$ and the columns are the $(x',z')$ corresponding to input. The ordering is chosen such that each blog-diagonal structure corresponds to a fixed $x_i, x_j'$ grid location. Thus the block diagonal components of the matrices correspond to $K(x,z|x,z')$. We see that the matrix is indeed local.  Here $\gamma = \omega = 100$ and $\kappa = 1/100$.} 
\label{fig:nonlocal_kernel_diffusivity}
\end{figure}

\begin{figure}
  \centerline{\includegraphics[width=1\textwidth]{Figures/nonlocal_kernel.png}}% Images in 100% size
  \caption{A representation of the full diffusivity kernel corresponding to the case in Figure \ref{fig:nonlocal_local_diffusivity}. If the diffusivity was indeed local then each of the form matrices would only have a diagonal component. The x-y coordinate axis have been collapsed to a single index, hence the banded structure of the output. Thus the rows are the "output" axis corresponding to the $(x,z)$ of $K(x,z|x',z')$ and the columns are the $(x',z')$ corresponding to input. The ordering is chosen such that each blog-diagonal structure corresponds to a fixed $x_i, x_j'$ grid location. Thus the block diagonal components of the matrices correspond to $K(x,z|x,z')$. Each block row looks similar since the turbulent flux should be the same at each grid point $x$. Within a block row we see a correlation patter for the contribution to the turbulent flux pattern depending on whether or not a given point is ``upstream" or ``downstream". The local diffusivity estimate sums over the $(x',y')$ axis to reduce it solely to a local diffusivity.  Here $\gamma = \omega = 1$ and $\kappa = 1$.} 
\label{fig:nonlocal_kernel_diffusivity}
\end{figure}


\begin{figure}
  \centerline{\includegraphics[width=1\textwidth]{Figures/nonlocal_kernel_symmetric.png}}% Images in 100% size
  \caption{A representation of the full diffusivity kernel. If the diffusivity was indeed local then each of the form matrices would only have a diagonal component. The x-y coordinate axis have been collapsed to a single index, hence the banded structure of the output. Thus the rows are the "output" axis corresponding to the $(x,z)$ of $K(x,z|x',z')$ and the columns are the $(x',z')$ corresponding to input. The ordering is chosen such that each blog-diagonal structure corresponds to a fixed $x_i, x_j'$ grid location. Thus the block diagonal components of the matrices correspond to $K(x,z|x,z')$. Each block row looks similar since the turbulent flux should be the same at each grid point $x$. Within a block row we see a correlation patter for the contribution to the turbulent flux pattern depending on the desitance from a given location $|x-x'|$. The local diffusivity estimate sums over the $(x',y')$ axis to reduce it solely to a local diffusivity.  Here $\gamma = 1$, $\omega = 0$ and $\kappa = 1$. } 
\label{fig:nonlocal_kernel_diffusivity}
\end{figure}


Thinking of a few limits. Here we take $T \rightarrow \infty$ first. If we then take $\gamma \rightarrow 0$ we see that the answer is different than commuting the limits. For example, $\gamma \rightarrow 0$ first would break the ergodicity assumption. Every initial velocity field would correspond to a "statistically steady state". Thus the turbulent-diffusivity and the conditional averages would all be different in that case. Ergodicity renders $P_m$ unique. Let, $\lambda_1$ be the smallest nonzero eigenvalue of the transition matrix. Then as long as $T \lambda_1 \rightarrow \infty$ as $T \rightarrow \infty$ and $\lambda_1 \rightarrow 0$ then one may expect the statistically steady state to be relevant. $\gamma \rightarrow \infty $ means that there are very rapid transitions between states. We see that if transitions are rapid, things are more local. The interpretation is that if a statistical trajectory spends sufficient time around a given state, one can expect it to pick up some nonlocal properties. It's worth noting that the strength of the turbulent-diffusivity is inversely proportional to diffusivity in the system. What's the takeway? The strength of the turbulent-flux can be suppressed by numerical dissipation.

Constructing states: How long on average does it take to get back to (roughly) where you started? This will (in general) depend on where you start and what your criteria is for being "roughly" in the same area. Start somewhere. Define distance criteria. Move until "distant". Pick up new state. Keep doing this for a while. Cluster new states. With operator splitting we can approximate things as locally linear at each timestep.perhaps small scales adjust quickly and large scales adjust slowly?

The Conditional Mean Equations are 
\begin{align}
\partial_t P_1 &= - \gamma P_1 + \frac{\gamma + \omega}{2}  P_2  +  \frac{\gamma - \omega}{2}  P_4 \\
\partial_t P_2 &= - \gamma P_2 + \frac{\gamma + \omega}{2}  P_3  +  \frac{\gamma - \omega}{2}  P_1 \\
\partial_t P_1 &= - \gamma P_3 + \frac{\gamma + \omega}{2}  P_4  +  \frac{\gamma - \omega}{2}  P_2 \\
\partial_t P_1 &= - \gamma P_4 + \frac{\gamma + \omega}{2}  P_1  +  \frac{\gamma - \omega}{2}  P_3 \\
 \partial_t \Theta_1 + \bm{u}_1 \cdot \nabla \Theta_1 
 &= D\Theta_1 + s P_1 - \gamma \Theta_1 + \frac{\gamma + \omega}{2}  \Theta_2  +  \frac{\gamma - \omega}{2}  \Theta_4 
 \\
 \partial_t \Theta_2 + \bm{u}_2 \cdot \nabla \Theta_2 
 &= D\Theta_2 + s P_2 - \gamma \Theta_2 + \frac{\gamma + \omega}{2}  \Theta_3  + \frac{\gamma - \omega}{2}  \Theta_1 
 \\
 \partial_t \Theta_3 + \bm{u}_3 \cdot \nabla \Theta_3 
 &= D\Theta_3 + s P_3 - \gamma \Theta_3 + \frac{\gamma + \omega}{2} \Theta_4   + \frac{\gamma - \omega}{2} \Theta_2  
 \\
 \partial_t \Theta_4 + \bm{u}_4 \cdot \nabla \Theta_4 
 &= D\Theta_4 + s P_4 - \gamma \Theta_4 + \frac{\gamma + \omega}{2} \Theta_1   + \frac{\gamma - \omega}{2}\Theta_3 
\end{align}
